Improving Shift Invariance in Convolutional Neural Networks with Translation Invariant Polyphase Sampling

Downsampling operators break the shift invariance of convolutional neural networks (CNNs) and this affects the robustness of features learned by CNNs when dealing with even small pixel-level shift. Through a large-scale correlation analysis framework, we study shift invariance of CNNs by inspecting existing downsampling operators in terms of their maximum-sampling bias (MSB), and find that MSB is negatively correlated with shift invariance. Based on this crucial insight, we propose a learnable pooling operator called Translation Invariant Polyphase Sampling (TIPS) and two regularizations on the intermediate feature maps of TIPS to reduce MSB and learn translation-invariant representations. TIPS can be integrated into any CNN and can be trained end-to-end with marginal computational overhead. Our experiments demonstrate that TIPS results in consistent performance gains in terms of accuracy, shift consistency, and shift fidelity on multiple benchmarks for image classification and semantic segmentation compared to previous methods and also leads to improvements in adversarial and distributional robustness. TIPS results in the lowest MSB compared to all previous methods, thus explaining our strong empirical results.

==> tables/cnn_vs_vit.tex <==
\begin{table}[t]
\centering
\Huge
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Invariance} & \textbf{CIFAR-10}   & \textbf{CIFAR-100} & \textbf{Food-101} & \textbf{Oxford-102} & \textbf{Tiny ImageNet} & \textbf{ImageNet} \\ 
\midrule
\textbf{Standard Shift} & 3.30 & 1.56 & 1.11 & 1.75 & 4.41 & 4.67 \\ 
\textbf{Circular Shift} & 3.23 & 1.56 & 0.48 & 2.11 & 4.92 & 4.67 \\ 
\bottomrule
\end{tabular}
}
\caption{
Relative performance improvement (\%) on image classification achieved by the most shift invariant ViT compared to the most shift invariant CNN model, both in terms of standard shift consistency and circular shift consistency.
}
\label{tab:cnn_vit}
\end{table}
